Enabling AI in Future Wireless Networks: A Data Life Cycle Perspective

Recent years have seen rapid deployment of mobile computing and Internet of Things (IoT) networks, which can be mostly attributed to the increasing communication and sensing capabilities of wireless systems. Big data analysis, pervasive computing, and eventually artificial intelligence (AI) are envisaged to be deployed on top of the IoT and create a new world featured by data-driven AI. In this context, a novel paradigm of merging AI and wireless communications, called Wireless AI that pushes AI frontiers to the network edge, is widely regarded as a key enabler for future intelligent network evolution. To this end, we present a comprehensive survey of the latest studies in wireless AI from the data-driven perspective. Specifically, we first propose a novel Wireless AI architecture that covers five key data-driven AI themes in wireless networks, including Sensing AI, Network Device AI, Access AI, User Device AI and Data-provenance AI. Then, for each data-driven AI theme, we present an overview on the use of AI approaches to solve the emerging data-related problems and show how AI can empower wireless network functionalities. Particularly, compared to the other related survey papers, we provide an in-depth discussion on the Wireless AI applications in various data-driven domains wherein AI proves extremely useful for wireless network design and optimization. Finally, research challenges and future visions are also discussed to spur further research in this promising area.

==> Application_Opportunities.tex <==
\section{Application Opportunities from BEoT paradigm }
\label{Sec:Application_Opportunities}
This section presents the application opportunities from BEoT paradigm via some key benefits.
\subsection{Smart transportation }
\subsection{Smart city}
\subsection{Smart healthcare}
\subsection{Smart agriculture }
\subsection{Smart home}


==> Challenges_Future-Directions.tex <==
\section{Challenges and Future Directions}
\label{Sec:Challenges_Future-Directions}
This section presents the key challenges and future directions related to BEoT research.
\subsection{Challenges} 
\subsubsection{Security in blockchain}
\subsubsection{Standardization}
\subsubsection{Resource management in BEoT}

\subsection{Future Directions} 
\subsubsection{Integrate AI with BEoT}
\subsubsection{BEoT in 5G}


	


==> Conclusion.tex <==
\section{Conclusion} 
\label{Sec:Conclusion}
In this article, we have conducted an extensive survey of the blockchain and Edge of Things integration. We have first introduced the overview of the blockchain and Edge of Things and discussed the main motivations behind the BEoT integrations. Furthermore, we have also provided a generic BEoT architecture where IoT, edge computing, blockchain and inherent applications and security services have been analysed. Next, we have paid attention to the review of the BEoT adoption in a number of important industrial applications, including smart transportation, smart city, smart healthcare, smart home, and smart grid. The security benefits of the BEoT paradigm have been discussed, with some key services such as access authentication, data privacy preservation, attack detection, and trust management. Finally, we have outlined some research challenges and pointed out open research directions toward BEoT-5G networks. We believe that this article will shed new lights on the BEoT research for future applications and services. 

==> Introduction.tex <==
\section{Introduction}
\label{Sec:Introduction}
In recent years, we have witnessed the rapid advances of Internet of Things (IoT) empowered by the proliferation of mobile devices such as smartphones, laptops, sensors, wearables, etc. It is predicted that by 2030, the number of connected IoT devices surpasses 500 million \cite{d1}. This tremendous expansion of IoT is expected to create numerous applications and services across different application domains, from industries, entertainments, to mobile games and surveillance \cite{d2,d3,d4}. Such IoT applications often require high computing resources to handle massive data generated from sensor devices with latency requirements to provide time-sensitive customer services, i.e., smart transportation, smart healthcare. Cloud computing can support IoT devices in solving computation tasks, but it remains high transmission latency due to long distance to the users. Edge computing has been recently proposed to support IoT with the creation of Edge of Things networks, by migrating computing and storage to the edge of the network, i.e., access points or base stations of radio access networks \cite{d5}, \cite{d6}. In this regard, the computational pressure burden posed on resource-constrained IoT sensors can be eliminated and the communication overhead is significantly reduced while achieving high users' computation experience. Therefore, Edge of Things has the great potential to provide location-aware distributed IoT applications, in order to facilitate time-sensitive service delivery with reduced computation complexities \cite{d7}.  

Nevertheless, the distribution nature of Edge of things introduces new also security and privacy challenges. The migration of large-scale computing and storage services to the network edge create the possibility of security threats such as jamming to be launched to control the network or attack the resources at edge nodes \cite{d8}, \cite{d9}. Moreover, uploading data to the network edge also raise critical data privacy concerns such as data breaches, data attacks, data modifications. Recently, blockhain, a disruptive technology emerged in recent years, has been regarded as a promising solution to solve security and privacy issues in edge computing networks as well as empower the next generations of Edge of Things technology \cite{d17}, \cite{d12}. In particular, the convergence of blockchain and Edge of Things creates a novel paradigm called \textit{BEoT}, which reshapes and transforms the conventional edge-IoT networks for enabling newly exiting industrial and customer applications and services \cite{d10}, \cite{d11}. For example, BEoT has been used to provide secure smart city services such as reliable vehicular management and low-latency traffic control \cite{d20}. Further, BEoT has promoted smart healthcare analytics and IoT medical processing due to the large-scale computing and communication of Edge of Things and security capability of blockchain \cite{d21}. The convergence of these emerging technologies is potentially a key enabler for future services and applications. 

\begin{figure*}
	\centering
	\includegraphics[height=14cm, width=18cm]{Images/Overview1.pdf}
	\caption{The generic architecture of BEoT.}
	\label{Fig:Overview}
\end{figure*}
\subsection{BEoT Architecture}
In this article, we propose a novel BEoT architecture that is enabled by the integration of blockchain and Edge of Things, as illustrated in Fig.~\ref{Fig:Overview}. The proposed architecture consist of three main entities, including Internet of Things, edge computing, blockchain, along with industrial applications and BEoT security services. 
\begin{itemize}
	\item \textit{Internet of Things (IoT):} IoT devices such as sensors, mobile phones are responsible for generating or gathering data from the physical environments and then transmit to the nearby edge servers via access points or base stations. IoT devices with certain resources (i.e., smart phones, laptops) can act as a mobile blockchain entity to make transactions in order to communicate directly with the edge servers or even join the blockchain mining for extra profits \cite{d13}. Other lightweight IoT devices such as sensors can participate in the blockchain network via their representative gateways (i.e., mobile phones) or other mobile blockchain entities in its IoT network \cite{d14}. 
	\item \textit{Edge computing:} In BEoT networks, IoT devices can offload their data to the edge servers (ESs) located at the base stations for processing. ESs are always equipped with rich computing and storage resources to handle IoT data tasks and provide data services for end users, ranging from data analytics, data prediction to data mining and data storage \cite{d15}, \cite{d16}. Moreover, each ES can also work as a blockchain miner that aims to verify the transactions and produce data blocks for maintaining the blockchain network. 
	\item \textit{Blockchain:} Blockchain is created to form the BEoT system running on top of the Edge of Things network, aiming to interconnect IoT devices, edge servers and end users together in a decentralized fashion. Particularly, blockchain is able to guarantee the reliable operations of BEoT systems without the need of a central authority or third-party, by using some key services such as data consensus, smart contracts, and shared ledgers \cite{d18}. 
	\item \textit{Industrial applications:} BEoT can enable new industrial applications thanks to the integration of blockchain and Edge of Things. For example, in a BEoT-based smart transportation system, the secure data analytic services at the edge vehicular servers (i.e., road side units) under the management of blockchain can support fast traffic control and reliable vehicle routing tasks even in the untrusted vehicular environment \cite{d19}. In the following sections, we discuss comprehensively the use of BEoT in various industrial applications, from smart transportation, smart city, smart healthcare to smart home and smart grid. 
	\item \textit{Security services:} Enabled by the inherent security properties such as decentralization, immutability, and traceability, blockchain can provide a number of important security services for BEoT, including access authentication, data privacy, attack detection, and trust management. The analysis of such security services will be presented in details later. 
\end{itemize}
\subsection{Comparisons to Other Related Works and Our Contributions}
In the literature, many studies in blockchain and Edge of Things topics have been investigated and conducted. The works in \cite{d22,d23,d24} presents extensive surveys on the integration of blockchain  and IoT from the different perspectives, from technical concept, architectures to research challenges. The potential of blockchain in enabling IoT applications and services has been also investigated in \cite{d25}. Moreover, the possibility of combining blockchain and edge computing has been investigated and surveyed in \cite{d26}, \cite{d27}. The survey in \cite{d28} paid attention to the discussion the roles of blockchain in edge computing architectures and several important applications of the integrated blockchain-edge computing model have been presented.  More recently, the convergence of blockchain and cloud computing, an extended paradigm of edge computing, has been discussed in recent survey papers \cite{d29}, \cite{d30}. 

Despite these much research efforts, we have found that a comprehensive review on the integration of blockchain and Edge of Things is still missing, to our best knowledge. Moreover, reviewing the state-of-the-art in the field, BEoT has increasingly attracted much interests in both academic and industry with a growing number of applied domains and use cases. Motivated by these, here we provide an extensive survey on the blockchain and Edge of Things integration, ranging from applications, opportunities to research challenges and future directions. The key objective of this article is to provide readers with the state-of-the-art knowledge of blockchain and Edge of Things and the recent advances in the BEoT technology. The key contributions of this survey are highlighted as follows.
\begin{enumerate}
	\item 	We provide a state-of-the-art survey on the blockchain and Edge of Things integration, starting with an updated discussion on the recent developments of blockchain and Edge of Things and highlighting the motivations of their combination. Moreover, a high-level BEoT architecture is also proposed and analysed. 
	\item 	 The key part of this article is focused on the opportunities of BEoT in industrial applications. In this regard, we present an in-depth survey on the use of BEoT in various important application domains, including smart transportation, smart city, smart healthcare, smart home, and smart grid. 
	\item 	Furthermore, security opportunities from the BEoT paradigm are also investigated. In particular, we analyze the benefits of blockchain in providing key security services for Edge of Things, such as access authentication, data privacy preservation, attack detection, and trust management. 
	\item 	Based on the extensive survey on the BEoT, we identify the potential research challenges and highlight some important future directions in BEoT.
\end{enumerate}
\subsection{Structure of The Survey}
The remainder of the article is organized as follows. Section II describes the state-of-the-art knowledge of blockchain and Edge of Things. The motivations of BEoT integration are also highlighted. In section III, we survey and analyze the recent development of BEoT technology in a wide range of industrial applications, including smart transportation, smart city, smart healthcare, smart home, and smart grid. The security opportunities brought by the BEoT paradigm are also presented and discussed in Section IV with some key services, such as access authentication, data privacy preservation, attack detection, and trust management. Section V provides some research challenges and outlines some possible future directions in the BEoT. Finally, Section VI concludes the paper.






==> Security_Opportunities.tex <==
\section{Security Opportunities from BEoT paradigm }
\label{Sec:Security_Opportunities}
This section presents the security opportunities from BEoT paradigm via some key benefits.
\subsection{Data privacy protection for Edge of Things}
\subsection{Attack detection for Edge of Things}
\subsection{Secure data management in Edge of Things}




==> State-of-Art.tex <==
\section{	State of the Art}
\label{Sec:State-of-Art}
This section presents the background and recent developments of blockchain, Edge of Things, and their combinations.
\subsection{Blockchain}

\subsection{Edge of Things}
\subsubsection{Mobile Edge Computing}
\subsubsection{Internet of Things}
\subsubsection{Edge of Things}
\subsection{Motivations of BEoT Integration}


